Not As Easy As You Think -- Experiences and Lessons Learnt from Trying to Create a Bottom-Up Visualization Image Typology

We present and discuss the results of a two-year qualitative analysis of images published in IEEE Visualization (VIS) papers. Specifically, we derive a typology of 13 visualization image types, coded to distinguish visualizations and several image characteristics. The categorization process required much more time and was more difficult than we initially thought. The resulting typology and image analysis may serve a number of purposes: to study the evolution of the community and its research output over time, to facilitate the categorization of visualization images for the purpose of teaching, to identify visual designs for evaluation purposes, or to enable progress towards standardization in visualization. In addition to the typology and image characterization, we provide a dataset of 6,833 tagged images and an online tool that can be used to explore and analyze the large set of tagged images. We thus facilitate a discussion of the diverse visualizations used and how they are published and communicated in our community.

==> BeforeMergeSection4.visTypes.tex <==
\section{Results and Discussion}
\label{sec:13vcs}
%\subsection{The Problem Domain}

Collaboratively coding these \imagesfigSeven led to many intensive discussions among the authors regarding our community design practices, the meaning of these types, dimensionalities, as well as the challenges we faced to characterize the images. 
%We also describe the classification of additional image attributes such as dimensionality, multiple compositions/views, and multiple nested or layered views. 
%\jc{commented out the multiple-view part.}
%\autoref{tab:12schema} provides an overview of the image categories we identified and defined. 
%In each subsection below,
In total we coded \imagesfigSeven images from the IEEE Visualization conference as discussed in \autoref{sec:process}. This process created \totaltypelabels visualization type labels, \totaldimlabels 2D/3D dimensionality labels, and \totalhardnesslabels hardness labels spread across the \imagesfigSeven 
images. Many images included several labels of different types. 
\autoref{fig:typeDistribution}
shows a distribution of the proportion of image labels in a category relative to the total images overlaid with the hardness ratings. 
%\autoref{fig:typeDistributionByDim}
shows the same image overlaid with the dimensions. 
\autoref{fig:typeDistributionByYear} gives a historic overview of the spread of types, dimensionality and hardness in a given year. 

%Here we describe each.
%Some of the categories are based on the four graphics primitives identified by Ward et al. \cite{Ward:2015:IDV} (points, lines, areas, and volumes), while we specified others based on other common patterns we observed. \tomo{this ref is misleading; Bertin referred already to points, lines, and areas; MacKinlay referred to volumes as well ... secondly, 
%we didn't specify other primitives on *that* level! our categories live on a very different conceptual ``dimension''!}

%Next we describe our 13 categories which necessitates a novel means to study what we see.\marginpar{\tiny\ms{does it?}} 
%We followed a simple coding rule, \ie, always to code  ``what you see'' rather than what you think the data is about. We also describe our definitions of their usage context such as dimensionality, multiple compositions/views, and multiple nested or layered views. 

%and GUIs are not necessarily one visualization. 

%The categories are initially
%defined and then refined during the coding process. Table~\cite{} shows the categories roughly from easy to hard. Types in this section are ordered by their frequency in the seven years we coded.
%If an image contains multiple sub-images or layered representations check the primary representation type.
%Check 3D when there is at least one 3D cue.
%\subsection{The Social Level: Micro-expert-crowdsourcing for Macro-tasks}

%\subsection{Visualization Types}


\subsection{Image Types, Their Dimensions, and Hardness}

Out of \imagesfigSeven images, 6704 ($98.1\%$) included at least one type of visualization types. 
The ``Other'' category includes anything that did not fit in any other category in our typology. An image can contains labels in this category.
%We used this category to describe what we saw preferably without using comments about what the data is about but rather about what the encoding looks like. \tomo{that is true for all categories, no?} 
%We used this category to describe what we saw preferably without using comments about what the data is about but rather about what the encoding looks like that is not in the 13 types above. %\tomo{that is true for all categories, no?} 
Photos potentially without annotations or labels (otherwise, it would be a schematic) ($\approx 200$ times), 
tables ($\approx 70$ times), plain text such as code, algorithms, texts that do not belong to the \vistext category ($\approx 20$ times), infographics, 
models, and legends (often color legends). 
There were \totalagreetodisagree images that the two coders agreed to disagree. In these cases, we added both coders' codes in our analyses. In addition, 
the hardness scores (of three levels, easy, neutral, and hard) are grouped into four categories: both coders coded hard (two-hard), 
both coders coded easy (two-easy),
at least one coders coded hard (one-hard), and others (neutral cases). 
The dimensions are also grouped into three categories 2D, 3D, and others (2D and 3D combined, I cannot tell and its combinations to 2D and 3D.)

The most common image type was \visschematic (xx of all types) followed by \vissurface (xxx). \visschematic is not a visualization type per-se by definition and \visgui are home to these visualization types. 
When combining \visschematic and \visgui, we see 
\todo{XXX} images (\todo{$xxx\%$} of all images).



In the next section we now summarize the coding results and describe the 13 categories that we identified based on our \emph{what-we-see} strategy from the \totaltypelabels labels we collected from \imagesfigSeven images.
We provide examples with an emphasis on contrasting the differences between our definitions of these types. 
Examples drawn mostly from our coding are in the end of each subsection. All images are to be referenced using numerical order from left to right and are used with permission.





\subsection{Our Visualization Typology}

\subsubsection{Generalized Bar Charts}% (LENGTH)}% (Michael and Petra)}
\label{sec:vc.bar}
\input{VisTypes/1vc.bar.tex}

\subsubsection{Point-based Techniques}% (POINT)}% (Michael and Torsten) }
\label{sec:vc.point}
\input{VisTypes/2vc.point.tex}

\subsubsection{Line-based Techniques}% (LINE)}% (Torsten and Jian)}
\label{sec:vc.line}
\input{VisTypes/3vc.line.tex}

\subsubsection{Node-link Trees/Graphs, Networks, Meshes}% (NODE-LINK)}% (Torsten and Tobias)}
\label{sec:vc.nodelink}
\input{VisTypes/4vc.nodelink.tex}

\subsection{Generalized Area Chart}% (AREA)}% (Tobias and Petra)}
\label{sec:vc.area}
\input{VisTypes/5vc.area.tex}

\subsubsection{Surface-based Techniques and Volumes}% (SURFACE)}% (Han-Wei and Torsten)} 
\label{sec:vc.surfacevolume}
\input{VisTypes/6vc.surfacevolume.tex}

\subsubsection{Generalized Matrix or Grid}% (GRID)}% (Tobias and Michael)}
\label{sec:vc.grid}
\input{VisTypes/7vc.grid.tex}

\subsubsection{Continuous Pattern-based Visualization}% (PATTERN)}% (Bob and Han-Wei)}
\label{sec:vc.pattern}
\input{VisTypes/8vc.pattern.tex}

\subsubsection{Continuous Color-based Encoding}% (COLOR)}% (Torsten and Bob)}
\label{sec:vc:color}
\input{VisTypes/13vc.color.tex}


\subsubsection{Glyph-based Techniques}% (GLYPH)}% (Petra and Bob)}
\label{sec:vc.glyph}
\input{VisTypes/9vc.glyph.tex}

\subsubsection{Text-based Encoding}% (TEXT)}% (Bob and Torsten)}
\label{sec:vc.text}
\input{VisTypes/11vc.text.tex}


\subsubsection{GUI (Screenshots)/User Interface Depiction}% (INTERFACE)}% (Petra and Michael)}
\label{sec:vc.gui}
\input{VisTypes/12vc.gui.tex}

\subsubsection{Schematic Representation, Images, Concept Illustrations}% (SCHEMATIC)}% (Michael and Tobias)}
\label{sec:vc.schematic}
\input{VisTypes/10vc.schematic.tex}

%\subsubsection{Others}% (OTHER)}% (Petra and Jian)}
%\label{sec:vc:other}
%\input{VisTypes/14vc.other.tex}

\subsubsection{\todo{Dimensionality: 2D and 3D}}
%\subsubsection{2D}
\label{sec:dim}

%\input{VisTypes/dim2d}
%\subsubsection{3D}
%\label{sec:dim3d}
%\input{VisTypes/dim3d}

\begin{comment}
\ms{should the following things be here or somewhere else? They are more about the actual coding process not so much about the actual typology. Or we label such things as ``\textbf{Additional coding remarks:}'' or so ...}

\subsection{Multiple Composition / Views (Juxtaposition)}
\label{sec:multicomposition}
\input{VisTypes/MultiComposition.tex}

\subsection{Multiple Nested, or Layered Views}
\label{sec:multinestedlayered}
\input{VisTypes/MultiNestedLayered.tex}

\end{comment}


==> BeforeMergeSection5.fuzzyCases.tex <==
%
% edited by RSL 28-29 March 2022
%
\section{Discussion: Challenges On Judging Visualization Types }
\label{sec:ambiguous}
%\label{sec:heuristics}

%VASTJ.280.1 \visglyph~\cite{cao2015targetvue}
%InfoVisC.195.3 \visnodelink and \visglyph~\cite{allendoerfer2005adapting}

%Representation, 
%Heuristics and Conflicts

This section presents together several challenging cases and the judgment heuristics we encountered during the coding process.
These borderline cases may span multiple categories. 
Ambiguous cases are much more common than we thought and are not difficult to imagine, 
\eg, What if a point, line, or an edge is used to encode a 1D length or height instead of a bar (chart)? or
\eg, How many data attributes need to be encoded in order for a visual design to be classified as a glyph?
Oftentimes, two (or more) visual designs may be combined in an attempt to inherit the benefits of both or inspire 
innovation.
%Because we cite many examples from articles and we put them in the supplemental materials.
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
The discussions over a two year period were at times akin to assessing the resemblance of an image with multiple visual designs: 
\textit{To what degree does X ``looks like'' Y?} It was often difficult to separate our perception from our domain knowledge and expertise.

%Several challenges encountered in the coding process are worth discussing. 

%\begin{figure}[!t]
%\centering
%\write18{wget \href{https://web.cse.ohio-state.edu/~chen.8028/VisPubImages/Images/2010/VisJ.1216.3.jpg}}
%\includegraphics{VisJ.1216.3.jpg}
%\includegraphics[width=\columnwidth]{\href{https://web.cse.ohio-state.edu/~chen.8028/VisPubImages/Images/2010/VisJ.1216.3.jpg}}%
%\label{fig:areahp}
%\caption{tttt}
%\end{figure}


% The following cases are not COLOR: (1) grid (representing a discrete colorspace); (2) discrete data (which should be grid), 
% and (3) categorical colormaps (which are chosen by the authors and can be replaced by any other maps).

%At a conceptual level, COLOR is not an discrete object and thus was not featured in our initial list categories. 

% Heatmap: typically, every element shows at pixel level computed from a constant function. For example, the color 
% progress is identical along the plane. The density of points is also a heatmap since the areas can appear darker or 
% lighter. 
% Heatmap is not surface-based coding because the surface does not capture the essential function or priority of the 
% visual channel.
% 2D medical images are heatmap because they change the intensity.


\subsection{What Types Should be in our Typology}

\textbf{Bertin's marks and channels as an inspiration.}
Bertin's theory~\cite{bertin1983semiology} examines two critical aspects of any graphic: the visual mark per data sample 
(\eg, a dot in a scatterplot graph) and its position in the plane (where the dot is placed relative to the x-axis and y-axis that bound the graph). 
Using this constructive approach would result in numerous (low-level) codes per image, but would not describe the visual design within a single class. 
For example, a scatterplot would be coded as a point and a position. 
However, we were striving for higher-level abstractions categories that include both the graphical primitives used and the coordinate system. 
Still, Bertin's definition of channels and marks provides inspiration to derive a set of categories. 
%If we use the ``mark'' and ``channel'' level of representation organization, scatterplot would be a dot and a position. Then we would have arrived at a vocabulary that lacks clear distinctions and clusters between techniques, other than a large, disjoint collections of data, task, channels, and marks.
%The theory of sign was useful to design to map each data dimensions to things appearing on the paper plane; Our intent is to study visual understanding after the visual construction thus need to a visually-connected representations understood by viewers.
%because interpretation and reasoning by humans often utilize multi-sensory input to \textit{summary} properties. 
Hence, we developed a more ``general point based techniques'' category that covers scatterplot-like images. 
In this category, the visual mark of a point would be dominant, perceptually.% where points would be the visual mark. 

%There are also functional and structural types. At high-level we may also study their composition into real-world uses.  \tomo{unclear what is meant here}


\textbf{Is ``continuous color-based encoding'' a separate type?}
Perceptual channels such as size and position are some of the most essential channels used in almost every visualization. 
% Hence, they are not really discriminatory. 
The same holds true for ``color'' (with multiple perceptual dimensions, such as hue, saturation, and luminance).
%, color preferences are also wired into the human visual system~\cite{palmer2010ecological}. 
% Color influences a wide spectrum of human behaviors ranged from  ensemble encoding to scatterplots to flow field visualizations.
%Many data were mapped to color which represents an important aspect of visual experience.
However, while also almost all visualizations use some type of color component, many of us coded heatmaps as a distinct category and
%We originally had heatmaps, 
one of the most frequent author keywords. Heatmaps often arise as a two-dimensional display of a data matrix. That lead us to merge it into the grid category. Yet, there was a distinct behavior of \visgrid to represent a discrete color mapping. However, the continuous appearance of color was remarkable and all of us felt that it deserves a separate treatment. %Continuous data are usually manipulated by computer in some finite approximate form such as sampled data. 
%Patterns or larger and small values are represented by continuous colormaps.
But not all uses of continuous colormaps results in heatmaps. % and they are useful by the authors to facilitate in the process of recognizing meaningful patterns of associated data. Discrete colors show map regions. 
Hence, after many discussions, we decided to create a distinct category to recognise the use of continuous color maps. We felt that this category is distinct enough from all others and, perceptually, its use sticks out and grabs attention.

\textbf{Not using data types as categories.}
We tried to avoid using data types in our classification schema. 
We originally had a cartographic map category and choose to remove it because it was governed by data type and there were ambiguities. Since our principle approach was based on perceptual cues, we believe that \visarea encoding are the primary approach used here. Geospatial maps primarily show regional divisions of areas. Of course, there are exceptions.
Route maps, where lines indicate a direct route, are coded separately as \visline because the routes encode data. 
%Terrains and landscapes were not man-made.
%\subsection{Dashboard: Machine or Humans Multiple View Composition}
%Map as an area rather than a geometry.
%Munzner defined map as geometry (spatial)~\cite{munzner2014visualization}.
%We had an extensive discussion on both geospatial and cartographic techniques on whether or not they belong to its own category, like Munzner~\cite{munzner2014visualization}. 
%We choose not to since geospatial or cartographic data are data types. The fundamental techniques still use area. 
One dificulty was the distinction between a ``map'' (cartographical map) and a ``terrain'' (wireframe rendering). Being guided by visual appearance, such images could appear as ``generalized area'' or as a ``surface-based technique''.
%We also agreed that terrain surfaces can be be categorical. We chose to code areas whether they are generated or natural as long as the area encodes data. 

One very special case to be discussed are chain code diagrams. We ended up coding this as a node-link diagram or ``I do not know''. Most coders used ``node-link'' because of the explicit nodes and the links which encode the numbers in the table. However, others coded lines. We chose to leave cases like this to future work and at present agree-to-disagree with each other's choices.

Text-based encodings is the only excemption to our rule of not coding data-type. However, it is such an esoteric type, that we felt it was justified in that case.


\subsection{Multiple Types Ambiguity}

\textbf{Influenced by Part-Whole Relationships.}
In general, many visualizations show multiple visual encodings. We agreed to code multiple categories, if these categories would stand on their own and can be clearly made out. However, there were several cases where one could have coded several categories, but we did not. 
\tochange{For example, }



\textbf{Influenced by coders' expertise}
%~\cite{lohse1994classification}. 
Though we chose to judge the visuals without knowledge of the data nor the data type (we ignored the captions)
%what the data type is - or what the data is about (e.g., by reading the captions), 
coders' expertise played a major role to resolve ambiguities. At times, we knew the original papers, but for most cases of ambiguity, we believed to have a good idea of the intention of the encoding.
%especially when in most cases, we value of the functional value of the plots in terms of why a visualization is chosen.
In a sense, our decision of labeling an image depended not only on the structure but also the intended function of the visualization. % value of the points and lines/bars.
For example, scarf plots~\cite{somarakis2020visual} 
%\tomo{I am not sure about a good reference} 
are coded as bars rather than lines because the space between lines as bar lengths are more important than the lines themselves. They do not encode data per se, but are meant as a dividing line.
\tochange{Further, scarf plots were not coded as a \matgd because the underlying grid is used as a layout rather than being part of the ``data''.
}

At first, we also had a separate category of ``tensor glyph mark''. However, this required the knowledge of an affine transform applied to a basic shape. This could not, however, be concluded from pure perceptual observations. So, we scrapped this category.
\begin{comment}
%We also tried to define tensor glyph marks using shapes that can be transformed by simple affine transformations and decided that one has to know the paper to analyze the math transforms correctly. These transforms are not directly perceivable. 
\tomo{I am not sure about the intention of this sentence, it is not coming out. A possible interpretation: At first, we also had a separate category of ``tensor glyph mark''. However, this required the knowledge of an affine transform applied to a basic shape. This could not, however, be concluded from pure perceptual observations. So, we scrapped this category.}
\jc{updated.}
\end{comment}

%Horizon chart \wordimg{FigureVCExamples/areaContinous3.jpg}~\cite{saito2005two} uses area to show 2D cluster membership graphs.  \tomo{what's the point of this sentence?}

\textbf{Many images attempt to combine advantages in a hybrid approach.}

%\subsection{One Vis - Many Encodings}
%\textbf{Micro and Macro Scales}
%\textbf{Primary vs. secondary is not easy to decide.}

%\textbf{One vis or multiple vis is not always obvious.}


\subsection{\visschematic does not contain actual data}

\begin{figure}[!t]
\centering
\subfloat[\visschematic]{\includegraphics[height=0.16\columnwidth]{FigureVCExamples/VisC.27.6.jpg}
\label{fig:tensorglyphs}}
\subfloat[\visnodelink]{\includegraphics[clip, trim={0 50 1000 0}, height=0.16\columnwidth]{FigureVCExamples/VisC.67.10.jpg}
\label{fig:chaincode}}
%VisC.67.10; chain-coded visualization~\cite{maeder1990animation}


%\subfloat[GLYPH+COLOR]{\includegraphics[width=0.14\textwidth]{FigureVCExamples/garcke2000Con1.jpg}%
%\label{fig_first_case}}
%\hfil
%\subfloat[\visglyph]{\includegraphics[width=0.165\textwidth]{FigureVCExamples/InfoVisJ.881.13.jpg}%
%\label{fig:}}
%\hfil
%\subfloat[\viscolor]{\includegraphics[width=0.16\textwidth]{FigureVCExamples/InfoVisJ.881.14.jpg}%
%\label{fig:c}}

%\hfil
\caption{Examples of \visschematic show the challenges to code some cases.  (Image courtesy of (a)~\cite{}))}
\label{fig:schematicHard}
\end{figure}


A large category of figures consists of schematic diagrams. 
It is often challenging to differentiate between schematics (which may not show actual data) and a demonstration of a visual encoding technique. %other rendering of real-data (which would be classified by techniques).
Some borderline instances are hard to characterize due to the lack of  
context information, such as axis, labels, etc. %, or conceptual or real-world referents about information which a visualization should convey.
\begin{comment}
Some were in lack of ``internal identification'', the relevant dimensions of variation in the pictorial content and determine which visual dimension corresponds to which conceptual variable or scale. \tomo{I don't know what is meant here.}
\end{comment}
We also found that many figures simply did not
depict these scales deemed important by Bertin~\cite{bertin1983semiology} and Cleveland~\cite{cleveland1985elements}, 
making the identification dichotomous among coders.
These observations aligned with Cleveland's observations while
reviewing other scientific journals~\cite{cleveland1985graphical}. 

For schematic diagrams, we experimented with different coding guidelines, e.g., when removing arrows and lines, is the remainder still a schematic.
To the contrary, one could argue that schematic views are meant to express 
pedagogical concepts, \ie, the addition of arrows and labels to a visualization can also result in a schematic. Thus our simple guideline of ``removing arrows'' could defeat its purpose. 
%We also tried to cover part of the image to test if visualization remains schematic and choose yes if so. Doing so assembles one's ability to be able to retrieve critical information from visualizations (e.g., interfaces labeled with ABC would become schematic). \tomo{sorry, I must have missed this discussion or am misunderstanding. At any rate, I cannot improve the description.}

%\tomo{RSL: I wonder if this type of discussion belongs in Section 5 (instead of here).}
We agreed that the appearance of labels/annotations to explain a visualization does not automatically 
mean an image is a schematic. 
A heuristic is that \visschematic contains no underlying ``dataset'', is intended to be pedagogical, and is intended to illustrate a concept.
If the image is a clear visual representation of data or a photograph without the labels it is not a schematic.  
A small example chart (of ``real data'') can appear inside of a schematic view, but would not be coded separately by us. 

% An often simplified representation showing the appearance, structure, or workings of something; a schematic representation. These figures allow the viewer to understand the (abstract) concept behind a technique, an algorithm, a specific implementation, a concept, or an idea.

% Logical or conceptual diagrams
% Schematics
% Pedagogical or concept drawings that do not vary with data
% Flowcharts
% Process visualization
% Annotated photos with labels pointing to content
% Images of hardware setups with annotations to show what is what

% When NOT to label schematic: schematic vs. labels/annotations
% If the image is a clear visual representation of data or a photograph without the labels it’s not a schematic.

% If the schematic includes multiple different VIS examples and it’s just one schematic (e.g. not multiple schematics side by side) it’s not multiple views

% Frequent characteristics:
% Often no underlying “dataset” loaded
% Often do not vary with data
% May include small example dataset
% Intended to be pedagogical
% Intended to illustrate a concept

% Here we don't code the techniques inside of the figure. 

\begin{comment}
\begin{figure}[!t]
\centering
%\subfloat[\visarea]{\includegraphics[height=0.2\columnwidth]{FigureVCExamples/AreaNotGridHorizonPlot.jpg}
%\label{fig:area1}}
%\subfloat[\visnodelink and \visarea]{\includegraphics[width=0.43\columnwidth]{FigureVCExamples/InfoVisC.131.3.jpg}
%\label{fig:nodelinkarea}}
\subfloat[\visarea, \visline, and \visglyph]{\includegraphics[width=0.33\columnwidth]{FigureVCExamples/VASTC.81.7.jpg}
\label{fig:lineareaglyph}}
%\subfloat[\visarea]{\includegraphics[clip, trim={0 0 560 0},width=0.3\columnwidth]{FigureVCExamples/InfoVisJ.1129.7.jpg}
%\label{fig:area2}}
%\subfloat[\visarea]{\includegraphics[width=0.32\columnwidth]{FigureVCExamples/InfoVisC.233.11.jpg}
%\label{fig:area3}}
\caption{Example of as \visarea. 
(a) A horizon plot is a type of \visarea and we checked only \visarea as the primary encoding, even though the grid created clear cutoffs of the timeline\tochange{, whose encoding is still continuous overall.}
Image courtesy of  
Saito et al.~\cite{saito2005two}.
%InfoVisC.131.1  and .3
(b)  Overbye et al. ~\cite{overbye2000new},
%VASTC.81.7
(c) Klemm et al.~\cite{klemm20153d},
%InfoVisJ.1129.7
(d) Dork et al.~\cite{dork2010visual}, and
(e) Riehmann et al.~\cite{riehmann2005interactive}.
\textcopyright\ IEEE, used with permission.}
\label{fig:areas}
\end{figure}
\end{comment}


%Challenging cases of area charts:
%\begin{enumerate}
%\setlength\itemsep{0em}
%\item The chart is in reality lines and was placed here because of its resemblance to the proceeding chart on the second axis to show the proportion.
%\item Channels added to a map will be coded separately because they are pronounced to show other data. For example, dot maps is to present geographic distribution data will be coded as point-based. Pies added to the route map till be coded as areas.
%\item
%\tochange{Matrix columns and rows, when not aligned in maps, also use areas. Each region/shape area is a mark.}
%\end{enumerate}



\subsection{Glyphs need to Contain Multiple Attributes}

\begin{figure}[!t]
\centering
%\hfil
%\subfloat[\visline]{\includegraphics[width=0.16\textwidth]{FigureVCExamples/hedgehog.jpg}%
%\label{fig:l}}
%\subfloat[GLYPH+COLOR]{\includegraphics[width=0.14\textwidth]{FigureVCExamples/garcke2000Con1.jpg}%
%\label{fig_first_case}}
%\hfil
\subfloat[\visglyph]{\includegraphics[width=0.165\textwidth]{FigureVCExamples/garcke2000Con3.jpg}%
\label{fig:g}}
%\hfil
\subfloat[\viscolor]{\includegraphics[width=0.16\textwidth]{FigureVCExamples/garcke2000Con4.jpg}%
\label{fig:c}}

\subfloat[\visglyph and \viscolor]{\includegraphics[width=0.16\textwidth]{FigureVCExamples/garcke2000Con2.jpg}%
\label{fig:gc}}
%\hfil
%\subfloat[\vispattern]{\includegraphics[width=0.16\textwidth]{FigureVCExamples/garcke2000Con6.jpg}%
%\label{fig:fp}}
\subfloat[\visglyph and \vispattern]{\includegraphics[width=0.165\textwidth]{FigureVCExamples/garcke2000Con5.jpg}%
\label{fig:fgp}}
%\hfil
\caption{\textbf{\visline, \visglyph, or \viscolor}. Flow simulation results (Image courtesy of 
(a) Weiskopf et al.~\cite{weiskopf2005overview}, 
%Spot noise. Verma et al.~\cite{verma2000flow} and (b)--(f) Garcke et al.~\cite{garcke2000continuous}.)
}
\label{fig:flowcases}
\end{figure}


\begin{figure}[!t]
\centering
\subfloat[\visglyph]{\includegraphics[clip, trim={300 50 1180 0},height=0.3\columnwidth]{FigureVCExamples/InfoVisJ.1558.13.jpg}%
\label{fig:glyphOnly}}
\hfil
\subfloat[\visarea]{\includegraphics[height=0.3\columnwidth]{FigureVCExamples/InfoVisC.149.10.jpg}%
\label{fig:areaGlypharea}}
\hfil
\subfloat[\visglyph]{\includegraphics[height=0.3\columnwidth]{FigureVCExamples/InfoVisC.149.15.jpg}%
\label{fig:areaGlyphglyph}}
\caption{(a) signifies the regional differences thus is a type of \visarea  and (b) features starGlyph-like dimensional comparisons and thus is a type of \visglyph. 
%\jc{could we discuss (b) again please?}
(Image courtesy of (a) Bian et al.~\cite{bian2020implicit} and (b)--(c) Fanea et al.~\cite{fanea2005interactive}.)}
\label{fig:glyphOrArea}
\end{figure}


\visglyph are special visual encodings that are localized at a specific spatial location. In that sense they can be mixed up with point based techniques. However, throughout the history of the visualization community, glyphs always had a special place and required a special treatment. The challenge, however, is to figure out when  a point is a point and when it becomes a glyph.

Pioneers in our field have attempted to define \emph{glyph}. 
The current definitions either consider the number of attributes or the number of marks and do not draw clear boundaries between visualization types. Fuchs et al.\ defined data glyphs as 
``data-driven visual entities, which make use of different visual channels to encode multiple attribute dimensions''~\cite{fuchs2013evaluation}. 
Borgo et al.~\cite{borgo2013glyph}  followed Ward to define glyphs as ``a visual representation of a piece of data where the attributes of a graphical entity are depicted by one or more attributes of a data record''~\cite{ward2008multivariate}.
In all these definitions, line and stripe (both using position) and pie (using area), and profile glyphs (using areas) are 
also coded as glyphs~\cite{fuchs2013evaluation, ward2002taxonomy}. In our definition, a point must contain high-dimensional data to become a type of \visglyph~\autoref{fig:glyphOnly}.

Munzner's glyph definition is broad and requires multiple marks. 
However, the marks do not have to come from different data attributes. For example, in Munzner's definition, each bar in the single stacked bar chart~\wordimg{FigureVCExamples/Munzner7.5stackedBarAsGlyph.jpg} is a ``microglyph'' because it is a composite object from multiple (colorful) length marks.  
Munzner also named the Streamgraph~\wordimg{FigureVCExamples/MunznerStreamAreaAsglyph.jpg} a glyph. 
We treat it as \visarea in our classification because these lines are stacked together to form areas. 
%showing numerous data attributes, such as timelines and frequency (as layer height). 
%However, this is classified as a glyph by Munzner~\cite{munzner2014visualization}.
Compared to Munzner's general definition, our definition requires the marks to show more than simple lines, points, and areas. 
Adding a channel such as color (e.g., circle size and color showing a quantitative datum) does not match our category of \visglyph. 
%\jc{is this hedgehog coding correct? Our coding changed recently.}
\tochange{Therefore, the popular hedgehog approach~\cite{garcke2000continuous}, where the flow is visualized by directed line segments whose lengths represent the magnitude of the velocity, is also not a \visglyph, but \visline in our encoding.
}

\begin{figure}[!t]
\centering
%\subfloat[\visnodelink]{\includegraphics[height=0.28\columnwidth]{FigureVCExamples/InfoVisC.219.10.jpg}
%\label{fig:line}} %~\cite{phan2005flow}
%flow map layout
%\subfloat[\visnodelink and \visarea]{\includegraphics[height=0.28\columnwidth]{FigureVCExamples/InfoVisJ.881.13.jpg}%
%\label{fig:nodelinkarea}}
%\hfil
\subfloat[\visline and \visarea]{\includegraphics[clip, trim={650 500 680 0},height=0.28\columnwidth]{FigureVCExamples/InfoVisJ.881.14.jpg}%
\label{fig:linearea}}
%\hfil
%\subfloat[\visnodelink]{\includegraphics[height=0.25\columnwidth]{FigureVCExamples/VisC.235.4.jpg}%\cite{suits2000simplification} 
%\label{fig:mesh}}
\subfloat[\visnodelink and \vissurface]{\includegraphics[clip, trim={680 50 0 0},height=0.25\columnwidth]{FigureVCExamples/VisJ.1271.2.jpg}%
\label{fig:nodelinkSurface}}
\subfloat[\visline, \vispoint, and \vissurface]{\includegraphics[clip, trim={0 0 330 0},height=0.25\columnwidth]{FigureVCExamples/InfoVisJ.559.7.jpg}%bach2015time
\label{fig:linepointsurface}}
\caption{\visnodelink. Image courtesy of 
%(a) Phan et al.~\cite{phan2005flow}, 
(b)Suits et al.~\cite{suits2000simplification},
%--(d) 
(c) Bach et al.~\cite{bach2015time}
%(e)  (f) Bach et al.~\cite{bach2015time}
}
\label{fig:nodelinkMeshes}
\end{figure}



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Section6.newStudy.tex <==
\section{Validation and Utilities: A Validation Study and An AI Classifier}

\changes{
The explosion of image data in publications has the potential to foster more sophisticated and robust models and algorithms to index, retrieve, organize and interact with images and multimedia data. In this section, we provide empirical evidences to validate the accuracy of our definitions and data selection. We did a human study on labeling new images and compared those to our own coding. 
In the second study, we 
}

==> TableImagesKeywordsStat.tex <==
\label{sec:dataset}
\begin{table}[!htb]
  \caption{Number of papers/number of figures per year per conference track, and 
  percentage of papers with keywords ($\%$ w/ keyW) every five years from 1990--2020. In the keywords related analysis,
  we use data from 2000--2020 due to scarce data points in
  the first two years. 
  }
  \label{tab:paperfigures}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	m{0.1cm}%
	m{0.6cm}m{0.6cm}m{0.6cm}m{0.6cm}
	m{0.6cm}m{0.6cm}m{0.6cm}m{0.6cm}
	%*{8}{c}%
	}
  \toprule
   \rotatebox{90}{year} & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} & \rotatebox{90}{InfoVis} & \rotatebox{90}{InfoVis conf} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &  Sum & \rotatebox{90}{$\%$ w/ keyW} \\
  \midrule
'20 & 32/374 &        & 65/614 & & 51/469 & 10/109 & 160/1566 &  \\
'15 & 33/401 & 9/80   & 38/387 & & 33/308 & 14/113 & 127/1289 &  \\
'10 & 48/575 &      & 35/318 & &  & 26/190 &  109/1083 &  \\
'05 &  & 88/847 &  & 31/296 & & & 119/1143 &  \\
'00 &  & 73/675  &  & 20/137  &   &  & 93/812 & \\
'95 &  & 56/424  &  & 18/97 &   &  & 74/521\\
'90 &  & 52/426  &  &  &   &  & 52/426  \\
  \midrule
  \textbf{sum} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{--} &\\
  \bottomrule
  \end{tabu}%
\end{table}

==> ThinkingWithYourEyesPackages.tex <==

\usepackage[T1]{fontenc}% use always vector fonts if available

\usepackage{mathptmx}
\usepackage{times}
\renewcommand*\ttdefault{txtt}       

\usepackage{subfigure}
\setlength{\subfigtopskip}{0pt}

%% it is recomended to use ``\autoref{sec:bla}'' instead of ``Fig.~\ref{sec:bla}''
%\graphicspath{{figures/}{pictures/}{images/}{./}}

% where to search for the images
\usepackage{comment}
\usepackage{microtype}                 % use micro-typography (slightly more compact, better to read)
\PassOptionsToPackage{warn}{textcomp}  % to address font issues with \textrightarrow
\usepackage{textcomp}                  % use better special symbols
\usepackage{mathptmx}                  % use matching math font
\usepackage{times}                     % we use Times as the main font
\renewcommand*\ttdefault{txtt}         % a nicer typewriter font
\usepackage{cite}                      % needed to automatically sort the references
\usepackage{tabu}                      % only used for the table example
\usepackage{booktabs}                  % only used for the table example

\usepackage{hyperref}
\hypersetup{pdftex,
   pagebackref=true,
   pdfpagemode=UseNone,
   pdftitle={\@title},
   pdfauthor={\@author},
   pdfsubject={},
   pdfkeywords={},
   pageanchor=true,
   plainpages=false,       % for problems with page referencing
   hypertexnames=false,    % for handling subfigures correctly
   bookmarks=true,         % we want bookmarks
   bookmarksnumbered=false,% include the section numbers in the list
   bookmarksopen=true,     % In the list, display highest level only
   bookmarksopenlevel=3,   % display three levels of bookmarks
   pdfpagemode=UseNone,    % show just the page
   pdfstartview=Fit,       % defail page view is the whole page at once
   pdfborder={0 0 0},      % we don't want those silly boxes for links
   breaklinks=true,        % allow breaking links
   colorlinks=false,       % don't change coloring of links
   nesting=true,
   linktocpage}


\usepackage{microtype}                 % use micro-typography (slightly more compact, better to read)
\PassOptionsToPackage{warn}{textcomp}  % to address font issues with \textrightarrow
\usepackage{textcomp}                  % use better special symbols
\usepackage{mathptmx}                  % use matching math font
\usepackage{times}                     % we use Times as the main font
\renewcommand*\ttdefault{txtt}         % a nicer typewriter font
\usepackage{cite}                      % needed to automatically sort the references
\usepackage{tabu}                      % only used for the table example
\usepackage{booktabs}                  % only used for the table example

\usepackage{tabularx}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
%\usepackage[xcolor=dvipdf]{changes}
%\usepackage[xcolor=dvipdf, final]{changes}
\usepackage{graphicx}
\usepackage{comment}
\usepackage{multirow} 
\usepackage[table,xcdraw]{xcolor}
\usepackage{subcaption}
\usepackage{epstopdf}
\usepackage{amsmath}
\usepackage{array}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{spy,calc}
\usetikzlibrary{fit}
\usepackage{todonotes}
\usepackage{xcolor}
\usepackage{array}


\definecolor{Blue}{RGB}{65,105,225}
\definecolor{Red}{RGB}{220,20,60}
\definecolor{Orange}{RGB}{255,140,0}

\newcommand{\changes}[1]{\protect\textcolor{Blue}{#1}}
%\renewcommand{\changes}[1]{#1}
\newcommand{\changesR}[1]{\protect\textcolor{Blue}{#1}}
%\renewcommand{\changesR}[1]{#1}
\newcommand{\tochange}[1]{\protect\textcolor{Red}{#1}}
%\renewcommand{\changesR}[1]{#1}
\newcommand{\toremove}[1]{\protect\textcolor{Orange}{#1}}


\newcommand{\psize}{1in}
\newcommand{\phsize}{1.25in}
\newcommand{\myspace}{\vskip -2\baselineskip plus -1fil}
\newcommand{\myspaceS}{\vskip -5\baselineskip plus -1fil}
\newcommand{\myspaceSS}{\vskip -15\baselineskip plus -1fil}

\newcommand*\mybc[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle, fill= cyan, draw=cyan, text=white, inner sep=0.8pt] (char) {#1};}}
\newcommand*\mygc[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle, fill=black, draw=black, text=white, inner sep=0.8pt] (char) {#1};}}

\usepackage{microtype}

\usepackage{xspace}
\newcommand{\dataname}{VIS7Y\xspace}
\newcommand{\toolname}{VISTechNavigator\xspace}
\newcommand{\toolnameshort}{VTEN\xspace}
\newcommand{\imagesfig}{29,689\xspace}
\newcommand{\imagesvis}{13,393\xspace}
\newcommand{\imagesscivis}{3,231\xspace}
\newcommand{\imagesinfovis}{7,818\xspace}
\newcommand{\imagesvast}{5,104\xspace}

\newcommand{\dengimagesfig}{12,267\xspace}
\newcommand{\dengimagescap}{12,057\xspace}
\newcommand{\dengpaper}{1,397\xspace}

\newcommand{\imagesfigSeven}{6,831\xspace}
\newcommand{\papersSeven}{695\xspace}

\newcommand{\numbar}{99999\xspace}
\newcommand{\numpoint}{99999\xspace}
\newcommand{\numline}{9999\xspace}
\newcommand{\numnodelink}{9999\xspace}
\newcommand{\numarea}{9999\xspace}
\newcommand{\numsurfacevol}{9999\xspace}
\newcommand{\nummatrixgrid}{9999\xspace}
\newcommand{\numglyph}{9999\xspace}
\newcommand{\numschematic}{9999\xspace}
\newcommand{\numpattern}{9999\xspace}
\newcommand{\numtext}{9999\xspace}
\newcommand{\numUI}{9999\xspace}
\newcommand{\numcannottell}{9999\xspace}


% left fixed width:
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
 
% center fixed width:
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% flush right fixed width:
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

\usepackage{multirow} 
\usepackage[table,xcdraw]{xcolor}
\usepackage{array}
\usepackage{enumitem}
\usepackage{textcomp}
\usepackage[most]{tcolorbox}

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\newcommand{\eg}{e.\,g.}
\newcommand{\ie}{i.\,e.}

\usepackage{mwe,subcaption,tikz}
%\usepackage{subfigure}
\tikzset{boximg/.style={remember picture,red,thick,draw,inner sep=0pt,outer sep=0pt}}

==> VisTypes/14vc.other.tex <==


This category includes anything that did not fit in any other category in our typology. 
%We used this category to describe what we saw preferably without using comments about what the data is about but rather about what the encoding looks like. \tomo{that is true for all categories, no?} 
We used this category to describe what we saw preferably without using comments about what the data is about but rather about what the encoding looks like that is not in the 13 types above. %\tomo{that is true for all categories, no?} 
general photographs potentially without annotations or labels (otherwise, it would be a schematic) ($\approx 200$ times), 
tables ($\approx 70$ times), plain text such as code, algorithms, texts that do not belong to the \vistext category ($\approx 20$ times), infographics, 
models, and legends (often color legends). 
%Photos can depict 2D or 3D scenes, and were coded accordingly.
%All photos are not necessarily 2D.\ms{weird formulation. Clear to us but likely not the reader?}


==> VisTypes/Challenges.tex <==

Challenging cases of generalized bar chart:
\begin{enumerate}
\setlength\itemsep{0em}
    \item Boxplots give evidence to the statistical description, where line length is essential to understanding. The line in a dot-plot also represents stack-together points. These points are linearly mapped to the range. 
    \item
    If only the bar top is shown (e.g., point-plot and Boxplot), use line \& point. If bars are drawn, use bar \& point. 
\end{enumerate}


==> VisTypes/MultiComposition.tex <==

Images that show a composition of multiple charts in a way that facilitates communication or rapid comparisons in subfigures. It could be a number of different data fields, using numerous encoding channels such as positioning in the coordinate (x, y), size, color, shape and so on or many charts partitioning data into the same encodings in multiple charts

\subsubsection{Yes, manually-arranged (for the purpose of communication / publication)}
Images containing (labeled or unlabeled) sub-figures or insets on top of images. 
Callouts are manually arranged.

\subsubsection{Yes, machine-arranged (as part of the vis system/interface)}
The views are shown side-by-side as part of a visualization or visualization system. This may include multiple GUIs containing multiple visualizations or screenshots of a subset of a multi-view system.  The view often has its own widgets and GUI components. \ms{Frankly, I am still confused by this reasoning. I am not sure if I ad any situation in which I had multiple screenshots of a GUI that were machine arranged (multiple yes, but manually arranged). On the other hand, it still is not ``intuitive'' to me why we did not code multi-view GUIs as multi-view.}

\subsubsection{No (just one vis)}
When the view just has one visualization  but also single GUIs that might contain multiple windows / overlays as part of the same system.\ms{iirc the guideline was that every GUI (of a single tool) is automatically just one vis ... }
Also, if a schematic includes multiple different VIS examples and it is just one schematic (\eg not multiple schematics side by side) it is not multiple views.


==> VisTypes/MultiNestedLayered.tex <==
Images containing layered / superimposition (multiple vis on top of each other) or nested (one vis representation inside another). Here the layered can mean the 2D/3D space or 2D/3D manifold space. 
It has at least two encoding techniques, such as wireframe mesh on top of a surface,
\eg, a cushion treemap (nested because of the shading and treemap together, not because of the containment relationships), 
painterly vector field (layered because of the vector glyph and the vorticity).

A single image
``multiple figures composed manually'' as a nested, \eg, call-out
subfigures containing a depiction of part of another subfigure
Containment relationships as nested due to data or algorithm, \eg, tree structures of a single encoding.
Small-multiples (they are “data dimensionality”, not “layout”)
Highlight or the photo category



==> VisTypes/dim3d.tex <==
3D representation has specific depth cues, such as shading, perspective, and lighting. It requires continous 3D, rather than discrete layers for aesthetics or callout uses. Here we ignore the media used to present the data. Thus a photo, a 3D data physicalization, and a desktop 3D interfaces can be 3D. 


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

